STAR-NT: Spatiotemporal Acceleration of Real-Time Neural Transparency Rendering

Neural order-independent transparency delivers high-quality rendering of overlapping transparent surfaces, but its geometry passes and network input generation remain costly, particularly on mobile and legacy hardware. We present a spatiotemporal acceleration framework that exploits spatial and temporal coherence to reduce this overhead while preserving visual quality. Spatially, we use adaptive quadtree-based screen-space subdivision to scale geometry pass resolution according to local color variance. Temporally, selected frames reuse the previous transparency result through depth-based reprojection instead of full rendering. Together, these optimizations reduce rendering cost and integrate efficiently into existing real-time rendering pipelines.

==> Tex/Implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}

Our method was specifically developed to accelerate DFAOIT~\cite{tsopouridis2024dfa}, providing both top-quality results and competitive performance.

All tile operations execute in compute shaders dispatched over a 2D grid of $8\times8$ thread groups. The quadtree state is maintained in a flat structured buffer of \texttt{uint3} records at 4 bytes per tile, with a second identically-sized buffer for double-buffered constraint enforcement. At $1920\times1080$ resolution, the tile grid occupies 33KB memory. Feature storage uses 16-bit per-channel textures throughout: two RGBA and two single-channel textures store the color and depth of the two peeled fragments, and two single-channel and one RGBA texture accumulate the remaining network input features. The total GPU memory footprint at $1920\times1080$ is approximately 75\,MB, identical to DFAOIT~\cite{tsopouridis2024dfa} under the same precision settings. For reference, WBOIT requires approximately 35.5MB, at the cost of the per-pixel fragment information that enables higher compositing accuracy. The neural network inference was implemented using fragment shaders.

Each geometry pass renders into a scaled render target determined by the tile complexity index $\bar{w}$ of the preceding frame (Sec.~\ref{adaptiveresolution}). Three target resolutions are maintained per pass (full, half, and quarter) are allocated at startup, avoiding runtime allocation. The inference pass always operates at full resolution, reading from upsampled copies of the scaled pass outputs. Shader source code is available online:\\ https://anonymous.4open.science/r/STAR-NT-8FC3/.
